Robust Detection Outcome: A Metric for Pathology Detection in Medical Images

Detection of pathologies is a fundamental task in medical imaging and the evaluation of algorithms that can perform this task automatically is crucial. However, current object detection metrics for natural images do not reflect the specific clinical requirements in pathology detection sufficiently. To tackle this problem, we propose Robust Detection Outcome (RoDeO); a novel metric for evaluating algorithms for pathology detection in medical images, especially in chest X-rays. RoDeO evaluates different errors directly and individually, and reflects clinical needs better than current metrics. Extensive evaluation on the ChestX-ray8 dataset shows the superiority of our metrics compared to existing ones. We released the code at https://github.com/FeliMe/RoDeO and published RoDeO as pip package (rodeometric).

==> Arxiv__Robust Detection Outcome/sections/00_abstract.tex <==
%auto-ignore
Detection of pathologies is a fundamental task in medical imaging and the evaluation of algorithms that can perform this task automatically is crucial.
However, current object detection metrics for natural images do not reflect the specific clinical requirements in pathology detection sufficiently.
To tackle this problem, we propose \emph{Robust Detection Outcome} (RoDeO); a novel metric for evaluating algorithms for pathology detection in medical images, especially in chest X-rays.
RoDeO evaluates different errors directly and individually, and reflects clinical needs better than current metrics.
Extensive evaluation on the ChestX-ray8 dataset shows the superiority of our metrics compared to existing ones. We released the code at \url{https://github.com/FeliMe/RoDeO} and published RoDeO as pip package (\texttt{rodeometric}).

==> Arxiv__Robust Detection Outcome/sections/01_intro.tex <==
%auto-ignore
\section{Introduction}\label{sec:intro}

% Motivation
Localization of pathologies in medical images is of high clinical relevance. It does not only speed up diagnosis but is also valuable to asses the interpretability of machine learning models.
Bounding boxes are especially useful in this regard, as they both satisfy the clinical need for coarse localization and are easier to obtain than exact segmentations.
However, assessing the quality of predicted bounding boxes is non-trivial. For object detection on natural images, metrics based on IoU-thresholds -- like \emph{Average Precision at IoU (AP@IoU)} or \emph{mean Average Precision (mAP)} -- are typically used.
We found these to be unsuitable for pathology detection in some medical images, such as chest radiographs.
%However, we have found current object detection metrics for natural images — like \emph{mean Average Precision (mAP)} — to be unsuitable for pathology detection in some medical images, such as chest radiographs.

% Explain AP@IoU and mAP briefly
The metric \emph{AP@IoU} first performs a greedy matching between predicted and target boxes while only considering predicted boxes that have the same class and an \emph{Intersection over Union (IoU)} above a defined threshold with the target box. Each target box can be matched to at most one predicted box (the one with the highest IoU). All unmatched boxes and those below the threshold are considered false positives. In the next step, the \emph{average precision (AP)} between the associated classes of the predicted and target boxes is computed. To obtain the mAP, the results of multiple IoU thresholds are averaged. % \footnote{In some cases, mAP is referred to as the AP at a single threshold only averaged over the classes. This is NOT the definition we use in this document.}.
% In the PASCAL VOC challenge \cite{pascal-voc-2007,pascal-voc-2012}, the IoU threshold is typically set to 0.5.
% To obtain the mAP, the results of multiple IoU threshold is averaged \footnote{In some cases, mAP is referred to as the AP at a single threshold only averaged over the classes. This is NOT the definition we use in this document.}. In COCO \cite{cocodataset}, thresholds in steps of 0.05 from 0.5 to 0.95 are used.
% Adding APs at such high thresholds favors models that have exact localizations. This is generally not clinically required.
Similarly, other classification metrics can be converted to detection metrics by computing them at IoU-thresholds, such as acc@IoU, recall@IoU, or precision@IoU (cf. Appendix \ref{sec:iou-based_metrics}).

% Clinical requirements
Although the tasks are similar, the requirements of object detection in natural images and pathology detection in medical images are much different.
For medical pathology detection, coarse localization is already clinically useful and the detection of pathologies is valuable even under misclassification since radiologists are well-trained to classify a pathology correctly once it is detected.
Lastly, different sources of detection errors need to be measured separately, a common requirement for all object detection tasks.
% Weaknesses of AP@IoU and mAP
Current object detection metrics do not reflect these requirements well:
IoU-based metrics are commonly used at high IoU-thresholds ($\geq0.5$). Since these are typically hard to obtain in pathology detection, and earlier works have used significantly lower thresholds \cite{nndetection,retinaunet}.
Additionally, these metrics do not differentiate between different types of errors: misclassification, faulty localization, box shape mismatch, and overprediction all cause false positives and thus degrade the score in the same way, although their underlying sources are much different. This makes metrics like AP@IoU hard to interpret and models hard to compare if they are only evaluated under this metric.
Moreover, AP@IoU and mAP are sensitive to misclassification and do not attribute the detection of pathologies if their predicted class is wrong.
Lastly, all metrics based on IoU thresholds only have a limited notion of proximity and drop harshly if the box overlap falls below the IoU-threshold.
Figure \ref{fig:example_boxes} shows cases where AP@IoU (and therefore also mAP) and acc@IoU exhibit such undesired behaviors.

% Weaknesses of AP@IoU and mAP
% Since coarse localization is oftentimes sufficient in pathology detection and high IoUs are typically hard to obtain, earlier works have used AP at significantly lower thresholds \cite{nndetection,retinaunet}, or have resorted to other flawed metrics, such as the accuracy or the average number of false positives at IoU (acc@IoU / afp@IoU) \cite{cxr8}.
% AP@IoU does further not differentiate between different types of errors: misclassification, faulty localization, shape mismatch, and overprediction all cause false positives and thus degrade the score in the same way, although their underlying sources are much different. This makes AP@IoU hard to interpret and different models hard to compare if they are only evaluated under this metric.
% Additionally, AP@IoU and mAP are very sensitive to misclassification and do not attribute the detection of pathologies if their predicted class is wrong. Though medical doctors are good at classifying pathologies once they are detected and can easily correct such errors.
% We also found that AP@IoU at low IoU thresholds can be tricked to produce reasonable performance with randomly placed bounding boxes (c.f. Section XY)


% How we do better
To tackle the aforementioned weaknesses of existing metrics, we introduce \emph{Robust Detection Outcome (RoDeO)}, a new metric for pathology detection based on
% five types of errors that cause the quality of an object detector prediction to deteriorate: classification errors, localization errors, shape mismatch, overprediction (more predictions than targets), and underprediction (less predictions than targets).
three types of errors that cause the detection quality to deteriorate: classification errors, localization errors, and shape mismatch.
RoDeO is easy to interpret, returns sub-scores for different error types, degrades gracefully, and reflects the specific requirements of pathology detection.

\paragraph{Our contributions are the following}
\begin{itemize}
    \item We identify weaknesses in current detection metrics when used for pathology detection.
    \item We propose RoDeO, a new metric for pathology detection that better reflects the clinical needs for course localization and separation of different error sources.
    \item We perform extensive evaluation of our proposed metric compared to existing ones and show that RoDeO is then only metrics capable of identifying weaknesses of an exemplary pathology detection model.
\end{itemize}


% Motivation to add
% - Medical images have much fewer boxes and positive classes than natural images (e.g. COCO)
% - Bounding boxes are sometimes ambiguous (Effusion)


==> Arxiv__Robust Detection Outcome/sections/02_related_work.tex <==
%auto-ignore
\section{Related Work}

% AP and mAP
The default metric for object detection in computer vision tasks is average precision. In the PASCAL VOC challenge \cite{pascal-voc-2007,pascal-voc-2012}, AP@50 is used, while in the COCO detection challenge \cite{cocodataset}, mAP is the main challenge metric (with IoU-thresholds from $0.5$ to $0.95$ in steps of $0.05$). Several attempts have been made to isolate different error types of AP@IoU and mAP by observing how the metric changes when certain errors in the predictions are fixed \cite{tide,borji2019empirical,hoiem2012diagnosing}. However, these techniques are merely fighting symptoms of average precision and inherit all other weaknesses of the metric minus its explainability. Moreover, they add another layer of complexity on top of the original metrics, again complicating their interpretability.
% \cite{tide} further have shown that fixing errors subsequently (as in \cite{borji2019empirical,hoiem2012diagnosing}) overestimates the influence of certain error types.
% Other IoU-based metrics
Recall@IoU -- or specifically the mean average recall over multiple IoU thresholds -- is also evaluated in the COCO detection challenge.
Other popular object detection metrics are also IoU-based. To evaluate a baseline model on the ChestX-ray8 dataset, \citet{cxr8} use the accuracy or number of average positive predictions at a given threshold \footnote{Wang \textit{et al.} chose the Intersection over Bounding Box (IoBB) instead of the IoU. This metric does not consider the size of the predicted box in the denominator and therefore favors large boxes.}.

% Overcoming IoU thresholds
All of the above metrics compute classification quantities after thresholding at an IoU. RoDeO overcomes this limitation and provides per-error metrics that are easily interpretable, degrade gracefully, and are tailored to clinical needs in pathology detection. %chest X-ray analysis.

Recently, \citet{metrics_reloaded} stressed the importance stressed the importance of adequate metric selection for the usefulness of machine learning algorithms in clinical practice.
While they acknowleddge that rough localization lies in the nature of object detection tasks, they only consider threshold-based metrics, such as AP
Our proposed metric follows their recommendation in first solving the assignment issue and then computing the selected metric on top, but we complement sole classification with other important factors, such as localization and shape correspondence.


==> Arxiv__Robust Detection Outcome/sections/03_metric.tex <==
%auto-ignore
\newcommand{\boxt}{\mathcal{B}^\mathfrak{t}}
\newcommand{\boxp}{\mathcal{B}^\mathfrak{p}}
\newcommand{\matchedp}{\mathcal{M}^\mathfrak{p}}
\newcommand{\matchedt}{\mathcal{M}^\mathfrak{t}}
\newcommand{\unmatchedp}{\mathcal{U}^\mathfrak{p}}
\newcommand{\unmatchedt}{\mathcal{U}^\mathfrak{t}}

\section{RoDeO Metric}
\paragraph{Overview}
In RoDeO, firstly one-to-one correspondences between the predicted and target bounding boxes are established. Then, three sub-metrics (localization, shape similarity, and classification) are computed using the matched boxes. The scores for over- and underpredictions are then linearly combined with the scores of each sub-metric.
Lastly, the harmonic mean of the three sub-metrics is computed to obtain one summary metric.


\paragraph{Matching}
To be able to compute subsequent sub-metrics, first, a matching between the predicted and target boxes is required for every image. We find these correspondences using the Hungarian method, taking into account correct classifications, as well as shape and distance information via the generalized IoU (gIoU) \cite{giou}.
Given the sets of target and predicted boxes, $\mathcal{M}^\mathfrak{t}$ and $\mathcal{M}^\mathfrak{p}$, the cost matrix $\mathcal{C}$ is:
\begin{equation}
    \mathcal{C}_{\boxt, \boxp} = -\mathds{1}_{[y_{\boxt}=y_{\boxp}]} * \omega_{cls} - \text{gIoU}(\boxt, \boxp) * \omega_{\text{shape}} \quad \forall \boxt \in \matchedt, \boxp \in{\matchedp} \,,
\end{equation}
with $\boxt$ and $\boxp$ being the boxes -- described by a vector $\left( x, y, w, h \right)^T$ -- and $y_{\boxt}$ and $y_{\boxp}$ being the classes of the target and predicted box respectively. $\omega_{\text{shape}}$ and $\omega_{\text{cls}}$ are parameters to weigh the importance of the two terms. By default, $\omega_{\text{shape}}$ is set to 1, and $\omega_{\text{cls}}$ is determined by the sample-wise classification performance of the predictions such that wrong class information does not confuse the matching when the model's class predictions are inaccurate.
We thus set $\omega_{\text{cls}} = \max\left(0, \text{MCC}\left(\bm{y}^\mathfrak{t}, \bm{y}^\mathfrak{p}\right)\right)$, where $y^\mathfrak{t}_i$ and $y^\mathfrak{p}_i$ are the classes of all target and predicted bounding boxes for image $i$, respectively, and 
$\text{MCC}$ is Matthews Correlation Coefficient \cite{mcc}, as defined in Eq.\ \eqref{eq:mcc} in Appendix \ref{appendix:definitions}.
This results in a set of matched boxes denoted by $\mathcal{M} = {(\boxp, \boxt) \mid \boxp \in \matchedp, \boxt \in \matchedt}$, where $(\boxp, \boxt)$ is a pair of matched bounding boxes. The set of unmatched targets is denoted by $\unmatchedt = \matchedt \setminus {\boxt \mid (\boxp, \boxt) \in \mathcal{M}}$, and the set of unmatched predicted bounding boxes is denoted by $\unmatchedp = \matchedp \setminus {\boxp \qquad \forall \, (\boxp, \boxt) \in \mathcal{M}}$.


\paragraph{Localization}
We measure the localization quality of the matched boxes in $\mathcal{M}$ by
\begin{align}
    \text{RoDeO}_\text{matched}^{\text{loc}} = \frac{1}{|\mathcal{M}|} \sum_{(\boxt, \boxp) \in \mathcal{M}}\exp\left[-\frac{\left(\frac{\boxt_x - \boxp_x}{\boxt_w}\right)^2 +\left(\frac{\boxt_y - \boxp_y}{\boxt_h}\right)^2}{C}\right] \,,
\end{align}
where $C$ is a scaling coefficient, set such that for a box pair $(\boxt, \boxp)$ with relative Euclidean distance equalling one, the value is exactly $0.5$, i.e.\ $\frac{1}{C} = \ln 2 \approx 0.69$.
The localization value for a single box pair thus follows the probability density of a (2D separable) normal distribution, such that (i) its maximum value is reached when box centers are aligned, (ii) it degrades slowly for small distances, then fast, until degrading slowly again for large distances.
Compared to IoU-based distance functions (used by acc@IoU, AP@IoU, or mAP), which degrade to zero very quickly and prefer axis-aligned boxes; $\text{RoDeO}_\text{matched}^{\text{loc}}$ degrades smoothly and isotropically in euclidean space, as highlighted in Figure \ref{fig:distance_metrics}.

\begin{figure}[h]
\floatconts
  {fig:distance_metrics}
  {\caption{Sensitivity of different metrics to position offsets. 
  For simplicity, we assume both, the target and predicted box, to be square and equal-sized. We plot the values of each metric with position offsets ($\Delta x = \frac{\boxt_x - \boxp_x}{\boxt_w}, \Delta y = \frac{\boxt_y - \boxp_y}{\boxt_h}$) between the predicted box and the target box (dashed box).
  %Note that if we assume a box size of 0.25 (approximately the average box size in the dataset used in this work), then the whole plot corresponds to a full image with the target box positioned in the center. 
  For mAP, we consider seven IoU-thresholds from 0.1 to 0.7.
  IoU-based distances (AP@50, mAP, IoU) degrade to zero very quickly and prefer axis-aligned boxes, while RoDeO loc degrades more smoothly and is isotropic in Eucledian space.
  }}
  {\includegraphics[width=\linewidth]{fig/distance_metrics.png}}
\end{figure}


\paragraph{Shape}
The shape score encodes differences in size and aspect ratio but must be independent of the distance between the boxes as this is already measured in the localization score. We compute it as the Intersection over Union (IoU) between each matched predicted and target box when assuming the boxes have the same center coordinates (cIoU):
%Shape similarity is computed as the Intersection over Union (IoU) between each matched predicted and target box when assuming the boxes have the same center coordinates (cIoU).
\begin{align}
    \text{RoDeO}_\text{matched}^{\text{shape}} = \frac{1}{|\mathcal{M}|} \sum_{(\boxt, \boxp) \in \mathcal{M}} \text{cIoU}(\boxt, \boxp) \,.
\end{align}
We refer to Appendix \ref{sec:design_decisions} for discussion on the preference of cIoU over alternative options.
% where cIoU is computed as the IoU after aligning the centers of predicted and target box.
%The shape score encodes differences in size and aspect ratio but must be independent of the distance between the boxes as this is already measured in the localization score.


\paragraph{Classification}
As classification score, RoDeO again uses $\text{MCC}$ (c.f. Equation \eqref{eq:mcc} in Appendix \ref{appendix:definitions}):
\begin{align}
    \text{RoDeO}_\text{matched}^{\text{cls}} = \max\left(0, \text{MCC}(\mathcal{Y}^\mathfrak{t}, \mathcal{Y}^\mathfrak{p})\right) \,,
\end{align}
where $\mathcal{Y}^\mathfrak{t} = \{ y_{\boxt} \}, \mathcal{Y}^\mathfrak{p} = \{ y_{\boxp} \} \qquad \forall ({\boxt}, {\boxp}) \in \mathcal{M}$, and $y_{\boxt}$ and $y_{\boxp}$ are the classes of the target and predicted box respectively.
In contrast to other classification metrics like F1-score or accuracy, MCC only gives positive scores for performance above random, regardless of possible class imbalances in the dataset. Since scores below $0$ indicate negative correlations, they should be valued the same as the outputs of completely random models.


\paragraph{Overprediction, Underprediction}
If over- and underpredictions (i.e. False Positives and False Negatives) are not penalized in the sub-metrics, these could be tricked by a large number of predictions. However, they can not be attributed to any of the aforementioned error types alone.
Instead, RoDeO integrates them globally into every sub-metric as a linear combination of the score achieved by the sub-metric and zero, weighted by the number of matched over- and underpredictions:
\begin{align}
    \text{RoDeO}^{\text{sub}} = \frac{|\mathcal{M}|}{|\mathcal{M}| + |\unmatchedt| + |\unmatchedp|} \text{RoDeO}_\text{matched}^{\text{sub}} \quad \forall \, \text{sub} \in \{  \text{loc}, \text{shape}, \text{cls} \} \,.
\end{align}
% \begin{align}
%     \text{RoDeO}^{\text{sub}} = \frac{\text{RoDeO}_\text{matched}^{\text{sub}} * m + \text{RoDeO}_\text{unmatched}^{\text{sub}} * (u^\mathfrak{t} + u^\mathfrak{p})}{m + u^\mathfrak{t} + u^\mathfrak{p}} \mid \text{sub} \in \{  \text{loc}, \text{shape}, \text{cls} \} \,,
% \end{align}
% where $m = |\mathcal{M}| * \omega_{matched}$, $u^\mathfrak{t} = |\unmatchedt| * \omega_{underpred}$, and $u^\mathfrak{p} = |\unmatchedp| * \omega_{overpred}$. 
% Depending on the requirements, the importance of each category can be adjusted via $\omega_{matched}$, $\omega_{underpred}$, and $\omega_{overpred}$, which are set to 1 per mid.

% Close duplicates of correct boxes are counted as negative. We deem it to be the responsibility of the model to filter multiple detections using established methods, such as weighted box fusion or non-maximum suppression.


\paragraph{Summary Metric}
We further propose a summarization of all the sub-metrics into a single number. We chose the harmonic mean (c.f.\ Appendix \ref{sec:design_decisions}) for aggregation because a low score in any sub-metric indicates a faulty detection algorithm that should not receive a high score in the summary metric. \emph{RoDeO total}, abbreviated \emph{RoDeO}, is thus computed as
\begin{align}
    \text{RoDeO} = 3 \left( \frac{1}{\text{RoDeO}^{\text{loc}}} + \frac{1}{\text{RoDeO}^{\text{shape}}} + \frac{1}{\text{RoDeO}^{\text{cls}}} \right)^{-1} \,.
\end{align}
% \begin{align}
%     \text{RoDeO} = \frac{3}{\frac{1}{\text{RoDeO}^{\text{loc}}} + \frac{1}{\text{RoDeO}^{\text{shape}}} + \frac{1}{\text{RoDeO}^{\text{cls}}}}
% \end{align}
% Nevertheless, we recommend laying the main focus on the sub-metrics when evaluating and comparing algorithms. The summary metric does not give a full picture of the different sources of errors.
Nevertheless, we recommend using the submetrics as well as the summary metric when measuring performance and comparing algorithms. The summary metric alone does not give a full picture of the different sources of errors.

\subsection{RoDeO per Class}
The computation of RoDeO on a per-class basis is analogous to above. However, for a class $c$, the set of matched boxes only contains the box pairs where the target box belongs to $c$.
% , i.e. $\mathcal{M}_c = \{ (\boxt, \boxp) \mid (\boxt, \boxp) \in \mathcal{M}, y_\boxt = c \}$.
The unmatched predicted and target boxes, are also filtered to the ones belonging to $c$. 
% $\unmatchedp_c = \boxp \mid \boxp \in \unmatchedp, y_\boxp = c$, and $\unmatchedt_c = \boxt \mid \boxt \in \unmatchedt, y_\boxt = c$



==> Arxiv__Robust Detection Outcome/sections/04_experimental_setup.tex <==
%auto-ignore
\section{Experimental Setup}
\paragraph{Dataset}
We perform experiments on the ChestX-ray8 dataset by \citet{cxr8}. It contains 108\,948 anterioposterior chest radiographs of 32\,717 unique patients acquired at the National Institutes of Health Clinical Center in the USA. The images are labeled for 8 different pathologies, each image can exhibit multiple pathologies. Additionally, a board-certified radiologist manually labeled 882 of these images with bounding boxes.
We used 50\% of the images with bounding boxes for evaluation and reserved the other 50\% for testing. The rest of the images were used for weakly-supervised training of a machine learning model. There was no patient overlap between all subsets.


\paragraph{Compared Metrics}
% Possible: AP@IoU, acc@IoU, afp@IoU, recall@IoU, TIDE
%In our experiments, 
We compare RoDeO to different threshold-based metrics: AP@IoU (the standard object detection metric for natural images) and acc@IoU \cite{cxr8}.
% as used in \cite{cxr8}, both at the thresholds $0.1$, $0.3$, and $0.5$.
% For these metrics, we look at three different IoU thresholds: $0.1$, $0.3$, and $0.5$. 
%, as is common practice on this dataset


\paragraph{Oracle Models and Prediction Corruption}
We study the sensitivity of object detection metrics, including RoDeO, to prediction quality changes and randomness using oracle models.
%To study how different object detection metrics, including RoDeO, react to differences in prediction quality and randomness, we experiment with oracle models on the test set.
These oracle models are not trained, but instead have access to the target boxes (i.e.\ the oracle) during inference. The correct bounding boxes are then modified using parameterized random corruption models before they are returned as predictions. We run these oracle models on the test set and study the effect of different corruptions and their parameters. For each corruption setting (with specified parameters), we report the mean results over five runs. We refer to Appendix \ref{appendix:corruption_models} for details on the corruption models.

\paragraph{CheXNet}
To test the usefulness of our proposed metric in practice, we train a CheXNet \cite{chexnet} as a weakly-supervised object detection model on the training dataset, using only image-level labels.
For the generation of bounding boxes from heatmaps, we follow \citet{cxr8}. Implementation details are provided in Appendix \ref{sec:implementation_details}.


==> Arxiv__Robust Detection Outcome/sections/05_experiment_results.tex <==
%auto-ignore
\section{Experiments}
In this section, we provide examples of undesired behavior of the compared metrics. In all cases, RoDeO behaves as expected. Further experimental results are shown in Appendix \ref{sec:additional_results}.

\paragraph{AP@IoU declines sharply with small localization errors.}
Figure \ref{fig:boxoracle_possizesigma} shows the influence of position- and size-corruptions on all compared metrics. While AP@IoU declines rapidly with position errors, it stays high under severe size corruptions. acc@IoU shows similar behavior but remains at a high base-value along all corruptions.
RoDeO declines more gracefully along both axes and shows a clear separation of the two corruptions.

\begin{figure}[h!]
\floatconts
  {fig:boxoracle_possizesigma}
  {\caption{RoDeO (bottom) declines more smoothly than acc@IoU (top left) and AP@IoU (top right) when position and shape are corrupted in our box oracle model. Position and shape corruptions are idenfitied independently by the RoDeO submetrics.}}
  % {\includegraphics[height=0.19\linewidth,trim={0 0 2.1cm 0},clip]{fig/plots_boxoracle/boxoracle_randcorrupt_relpossize_acc.png}
  % \includegraphics[height=0.19\linewidth,trim={0 0 2.1cm 0},clip]{fig/plots_boxoracle/boxoracle_randcorrupt_relpossize_AP.png}
  {\includegraphics[height=0.19\linewidth,trim={0 0 3.27cm 0},clip]{fig/plots_boxoracle/boxoracle_randcorrupt_relpossize_acc.png}
  \includegraphics[height=0.19\linewidth]{fig/plots_boxoracle/boxoracle_randcorrupt_relpossize_AP.png}
  \includegraphics[height=0.19\linewidth]{fig/plots_boxoracle/boxoracle_randcorrupt_relpossize_RoDeO.png}}
\end{figure}


\paragraph{Acc@IoU achieves high scores with underprediction.}
In Figure \ref{fig:boxoracle_undersample}, acc@50 increases with higher underprediction probability (i.e.\ more missed boxes). This leads to higher scores for models that predict no boxes at all, especially at higher IoUs.
With more underprediction, a higher number of false positives are exchanged with true negatives, leading to better accuracy.
AP@IoU and RoDeO do not suffer from this behavior.

\begin{figure}[h!]
\floatconts
  {fig:boxoracle_undersample}
  {\caption{
  Acc@IoU (left) increases with fewer predictions, whereas AP@IoU (middle) and RoDeO (right) decline as expected when corrupting the box positions ($\sigma_\text{pos}=0.5$) and randomly dropping predicted boxes ($p_\text{underpred}$) in our box oracle model.
  }}
  {\includegraphics[width=0.32\linewidth]{fig/plots_boxoracle/boxoracle_undersample_fixedsizesigma_acc.png}
  \includegraphics[width=0.32\linewidth]{fig/plots_boxoracle/boxoracle_undersample_fixedsizesigma_AP.png}
  \includegraphics[width=0.32\linewidth]{fig/plots_boxoracle/boxoracle_undersample_fixedsizesigma_RoDeO.png}}
\end{figure}


\paragraph{AP@IoU ignores overprediction at higher thresholds.}
While overprediction leads to an exponential decay (as expected) of all sub-metrics of RoDeO, AP@IoU does not decay with more overprediction at $\text{IoUs} > 10 \%$ in Figure \ref{fig:boxoracle_overperclass}. Even worse, AP@50 shows a small but significant increase as more boxes get predicted.

\begin{figure}[h!]
\floatconts
  {fig:boxoracle_overperclass}
  {\caption{AP@IoU (middle) at higher thresholds increases with more predictions. acc@IoU (left) and RoDeO (right) decline as expected when corrupting the box positions ($\sigma_\text{pos}=0.5$) and randomly predicting multiple boxes per target ($p_\text{overpred}$).}}
  {\includegraphics[width=0.32\linewidth]{fig/plots_boxoracle/boxoracle_overperclass_fixedsizesigma_acc.png}
  \includegraphics[width=0.32\linewidth]{fig/plots_boxoracle/boxoracle_overperclass_fixedsizesigma_AP.png}
  \includegraphics[width=0.32\linewidth]{fig/plots_boxoracle/boxoracle_overperclass_fixedsizesigma_RoDeO.png}}
\end{figure}

\subsection{Evaluating a Machine Learning Model}

\begin{table}[htb]
\floatconts
    {tab:chexnet}
    {\caption{Qualitative RoDeO, acc@30, and mAP results of a trained CheXNet model. For mAP, we consider seven thresholds from $0.1$ to $0.7$.}}
    {\resizebox{0.85\textwidth}{!}{\begin{tabular}{lcccccc}
    \toprule
                 & RoDeO/cls & RoDeO/loc & RoDeO/shape & RoDeO & acc@30 & mAP    \\
    \midrule
    Atelectasis  & 21.6      & 17.3      &  6.9        & 28.4  & 37.1   &  2.0    \\
    Cardiomegaly & 55.7      & 70.4      & 45.8        & 55.6  & 86.2   & 31.7    \\
    Effusion     & 21.9      & 15.5      &  9.2        & 13.7  & 33.4   &  5.1    \\
    Infiltration & 11.0      & 15.9      &  8.1        & 10.8  & 31.6   &  3.0    \\
    Mass         & 10.6      & 11.4      &  4.3        &  7.2  & 59.4   &  1.6    \\
    Nodule       & 16.9      &  3.0      &  0.8        &  1.9  & 55.7   &  0.0    \\
    Pneumonia    &  9.2      & 38.3      & 19.2        & 16.0  & 71.6   &  2.1    \\
    Pneumothorax & 26.6      & 14.3      & 12.5        & 16.0  & 65.8   &  1.0    \\
    Total        & 19.8      & 19.9      & 10.9        & 15.6  & 55.1   &  5.8    \\
    \bottomrule
\end{tabular}}}
\end{table}

Table \ref{tab:chexnet} shows qualitative results of RoDeO and mAP for a trained CheXNet \cite{chexnet}.
In mAP, atelectasis and pneumonia achieve similar scores, the results of RoDeO paint a more balanced picture.
While atelectasis is classified quite well, its predicted shape does often mismatch. For pneumonia, on the other hand, location and shape are predicted quite well, but it was rarely classified correctly by the model -- acc@IoU, however, gives one of the highest scores to pneumonia, which is due to the dominance of true negatives in accuracy and renders the metric almost completely useless.
RoDeO also reveals that the most severe problem in nodule detection is the shape (or size) mismatch followed by localization, while classification is comparably good.


==> Arxiv__Robust Detection Outcome/sections/06_discussion.tex <==
%auto-ignore
\section{Discussion}
The above experiments have shown that compared to IoU-based metrics (cf. Sec.\ \ref{sec:intro}), RoDeO has more desirable behaviors for medical object detection: It can not be tricked by over- or under-prediction, it does not consider boxes with class confusion as useless but values the detection of pathologies separately, and it uses a notion of distance that reflects the clinical need for coarse localization better.
Our experiments have further shown that different error sources affect sub-metrics independently and that RoDeO degrades gracefully along all sub-metrics.
Further evaluation in Appendix \ref{sec:additional_results} shows that RoDeO also behaves as desired in a plethora of different corruption settings.
While we have shown the usefulness of RoDeO for pathology detection, we argue that other medical object detection tasks, such as organ detection, could also benefit from the adavantages of RoDeO. %We leave such an analysis to future work.



==> Arxiv__Robust Detection Outcome/sections/07_conclusion.tex <==
%auto-ignore
\section{Conclusion}
We have proposed RoDeO, a novel metric to evaluate object detection algorithms, that is tailored to the requirements in medical pathology detection, especially from chest X-rays.
Extensive experiments have shown that RoDeO considers different error-sources more appropriately than previous metrics.
It is easy to interpret and use; with robust default values that can easily be adapted to the specific needs of an application.
RoDeO allows for better evaluation of pathology detection algorithms and can increase their clinical usefulness.

